The physical and chemical structure of Sagittarius B2 VIIIa. Dust and ionized gas contributions to the full molecular line survey of 47 hot cores

Sagittarius B2 (Sgr B2) is a giant molecular cloud complex in the central molecular zone of our Galaxy hosting several sites of high-mass star formation. The two main centers of activity are Sgr B2(M) and Sgr B2(N), which contain 27 and 20 continuum sources, respectively. Our analysis aims to be a comprehensive modeling of each core spectrum, where we take the complex interaction between molecular lines, dust attenuation, and free-free emission arising from HII regions into account. In this work, we determine the dust and, if HII regions are contained, the parameters of the free-free thermal emission of the ionized gas for each core, and derive a self-consistent description of the continuum levels of each core. Using the high sensitivity of ALMA, we characterize the physical and chemical structure of these continuum sources and gain better insight into the star formation process within the cores. We used ALMA to perform an unbiased spectral line survey of all 47 sources in ALMA band 6 with a frequency coverage from 211 GHz to 275 GHz. In order to model the free-free continuum contribution of a specific core, we fit the contained recombination lines (RRLs) to obtain the electron temperatures and the emission measures, where we use an extended XCLASS program to describe RRLs and free-free continuum simultaneously. In contrast to previous analyses, we derived the corresponding parameters here not only for each core, but also for their local surrounding envelope, and determined their physical properties. The distribution of RRLs we found in the core spectra closely fits the distribution of HII regions described in previous analyses. For the cores we determine average dust temperatures of around 236 K (Sgr B2(M)) and 225 K (Sgr B2(N)), while the electronic temperatures are located in a range between 3800 K and 23800 K.

==> figures/error/SgrB2-M/error-estimation__SgrB2-M.tex <==


%--------------------------------------------------------------------------------
% Error estimation

    \section{Error estimation}


%--------------------------------------------------------------------------------
% Error estimation of continuum parameters for cores in Sgr~B2(M)

    \subsection{Error estimation of continuum parameters for cores in Sgr~B2(M)}\label{app:ErrorSgrB2-M}

Corner plots \citepads{{corner}} showing the one and two dimensional projections of the posterior probability distributions of the continuum parameters of each core in Sgr~B2(M). On top of each column the probability distribution for each free parameter is shown together with the value of the best fit and the corresponding left and right errors. The left and right dashed lines indicate the lower and upper limits of the corresponding HPD interval, respectively. The dashed line in the middle indicates the mode of the distribution. The blue lines indicate the parameter values of the best fit. The plots in the lower left corner describe the projected 2D histograms of two parameters and the contours the HPD regions, respectively. In order to get a better estimation of the errors, we determine the error of the hydrogen column density and the emission measure on log scale and use the velocity offset (v$_{\rm off}$) related to the source velocity of v$_{\rm LSR}$ = 64~km~s$^{-1}$.


% core A01
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A01__env.pdf}\\
   \caption{Corner plot for source A01, envelope layer.}
   \label{fig:SgrB2-MErrorA01env}
\end{figure*}


% core A01
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A01__core.pdf}\\
   \caption{Corner plot for source A01, core layer.}
   \label{fig:SgrB2-MErrorA01core}
\end{figure*}
\newpage
\clearpage




% core A02
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A02__env.pdf}\\
   \caption{Corner plot for source A02, envelope layer.}
   \label{fig:SgrB2-MErrorA02env}
\end{figure*}


% core A02
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A02__core.pdf}\\
   \caption{Corner plot for source A02, core layer.}
   \label{fig:SgrB2-MErrorA02core}
\end{figure*}
\newpage
\clearpage




% core A03
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A03__env.pdf}\\
   \caption{Corner plot for source A03, envelope layer.}
   \label{fig:SgrB2-MErrorA03env}
\end{figure*}


% core A03
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A03__core.pdf}\\
   \caption{Corner plot for source A03, core layer.}
   \label{fig:SgrB2-MErrorA03core}
\end{figure*}
\newpage
\clearpage




% core A04
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A04__env.pdf}\\
   \caption{Corner plot for source A04, envelope layer.}
   \label{fig:SgrB2-MErrorA04env}
\end{figure*}


% core A04
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A04__core.pdf}\\
   \caption{Corner plot for source A04, core layer.}
   \label{fig:SgrB2-MErrorA04core}
\end{figure*}
\newpage
\clearpage




% core A05
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A05__env.pdf}\\
   \caption{Corner plot for source A05, envelope layer.}
   \label{fig:SgrB2-MErrorA05env}
\end{figure*}


% core A05
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A05__core.pdf}\\
   \caption{Corner plot for source A05, core layer.}
   \label{fig:SgrB2-MErrorA05core}
\end{figure*}
\newpage
\clearpage




% core A06
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A06__env.pdf}\\
   \caption{Corner plot for source A06, envelope layer.}
   \label{fig:SgrB2-MErrorA06env}
\end{figure*}


% core A06
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A06__core.pdf}\\
   \caption{Corner plot for source A06, core layer.}
   \label{fig:SgrB2-MErrorA06core}
\end{figure*}
\newpage
\clearpage




% core A07
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A07__env.pdf}\\
   \caption{Corner plot for source A07, envelope layer.}
   \label{fig:SgrB2-MErrorA07env}
\end{figure*}


% core A07
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A07__core.pdf}\\
   \caption{Corner plot for source A07, core layer.}
   \label{fig:SgrB2-MErrorA07core}
\end{figure*}
\newpage
\clearpage




% core A08
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A08__env.pdf}\\
   \caption{Corner plot for source A08, envelope layer.}
   \label{fig:SgrB2-MErrorA08env}
\end{figure*}


% core A08
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A08__core.pdf}\\
   \caption{Corner plot for source A08, core layer.}
   \label{fig:SgrB2-MErrorA08core}
\end{figure*}
\newpage
\clearpage




% core A09
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A09__env.pdf}\\
   \caption{Corner plot for source A09, envelope layer.}
   \label{fig:SgrB2-MErrorA09env}
\end{figure*}
\newpage
\clearpage




% core A10
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A10__env.pdf}\\
   \caption{Corner plot for source A10, envelope layer.}
   \label{fig:SgrB2-MErrorA10env}
\end{figure*}
\newpage
\clearpage




% core A11
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A11__env.pdf}\\
   \caption{Corner plot for source A11, envelope layer.}
   \label{fig:SgrB2-MErrorA11env}
\end{figure*}


% core A11
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A11__core.pdf}\\
   \caption{Corner plot for source A11, core layer.}
   \label{fig:SgrB2-MErrorA11core}
\end{figure*}
\newpage
\clearpage




% core A12
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A12__env.pdf}\\
   \caption{Corner plot for source A12, envelope layer.}
   \label{fig:SgrB2-MErrorA12env}
\end{figure*}


% core A12
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A12__core.pdf}\\
   \caption{Corner plot for source A12, core layer.}
   \label{fig:SgrB2-MErrorA12core}
\end{figure*}
\newpage
\clearpage




% core A13
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A13__env.pdf}\\
   \caption{Corner plot for source A13, envelope layer.}
   \label{fig:SgrB2-MErrorA13env}
\end{figure*}


% core A13
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A13__core.pdf}\\
   \caption{Corner plot for source A13, core layer.}
   \label{fig:SgrB2-MErrorA13core}
\end{figure*}
\newpage
\clearpage




% core A14
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A14__env.pdf}\\
   \caption{Corner plot for source A14, envelope layer.}
   \label{fig:SgrB2-MErrorA14env}
\end{figure*}


% core A14
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A14__core.pdf}\\
   \caption{Corner plot for source A14, core layer.}
   \label{fig:SgrB2-MErrorA14core}
\end{figure*}
\newpage
\clearpage




% core A15
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A15__env.pdf}\\
   \caption{Corner plot for source A15, envelope layer.}
   \label{fig:SgrB2-MErrorA15env}
\end{figure*}


% core A15
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A15__core.pdf}\\
   \caption{Corner plot for source A15, core layer.}
   \label{fig:SgrB2-MErrorA15core}
\end{figure*}
\newpage
\clearpage




% core A16
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A16__env.pdf}\\
   \caption{Corner plot for source A16, envelope layer.}
   \label{fig:SgrB2-MErrorA16env}
\end{figure*}


% core A16
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A16__core.pdf}\\
   \caption{Corner plot for source A16, core layer.}
   \label{fig:SgrB2-MErrorA16core}
\end{figure*}
\newpage
\clearpage




% core A17
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A17__env.pdf}\\
   \caption{Corner plot for source A17, envelope layer.}
   \label{fig:SgrB2-MErrorA17env}
\end{figure*}


% core A17
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A17__core.pdf}\\
   \caption{Corner plot for source A17, core layer.}
   \label{fig:SgrB2-MErrorA17core}
\end{figure*}
\newpage
\clearpage




% core A18
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A18__env.pdf}\\
   \caption{Corner plot for source A18, envelope layer.}
   \label{fig:SgrB2-MErrorA18env}
\end{figure*}
\newpage
\clearpage




% core A19
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A19__env.pdf}\\
   \caption{Corner plot for source A19, envelope layer.}
   \label{fig:SgrB2-MErrorA19env}
\end{figure*}


% core A19
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A19__core.pdf}\\
   \caption{Corner plot for source A19, core layer.}
   \label{fig:SgrB2-MErrorA19core}
\end{figure*}
\newpage
\clearpage




% core A20
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A20__env.pdf}\\
   \caption{Corner plot for source A20, envelope layer.}
   \label{fig:SgrB2-MErrorA20env}
\end{figure*}
\newpage
\clearpage




% core A21
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A21__env.pdf}\\
   \caption{Corner plot for source A21, envelope layer.}
   \label{fig:SgrB2-MErrorA21env}
\end{figure*}


% core A21
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A21__core.pdf}\\
   \caption{Corner plot for source A21, core layer.}
   \label{fig:SgrB2-MErrorA21core}
\end{figure*}
\newpage
\clearpage




% core A22
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A22__env.pdf}\\
   \caption{Corner plot for source A22, envelope layer.}
   \label{fig:SgrB2-MErrorA22env}
\end{figure*}


% core A22
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A22__core.pdf}\\
   \caption{Corner plot for source A22, core layer.}
   \label{fig:SgrB2-MErrorA22core}
\end{figure*}
\newpage
\clearpage




% core A23
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A23__env.pdf}\\
   \caption{Corner plot for source A23, envelope layer.}
   \label{fig:SgrB2-MErrorA23env}
\end{figure*}


% core A23
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A23__core.pdf}\\
   \caption{Corner plot for source A23, core layer.}
   \label{fig:SgrB2-MErrorA23core}
\end{figure*}
\newpage
\clearpage




% core A24
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A24__env.pdf}\\
   \caption{Corner plot for source A24, envelope layer.}
   \label{fig:SgrB2-MErrorA24env}
\end{figure*}


% core A24
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A24__core.pdf}\\
   \caption{Corner plot for source A24, core layer.}
   \label{fig:SgrB2-MErrorA24core}
\end{figure*}
\newpage
\clearpage




% core A25
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A25__env.pdf}\\
   \caption{Corner plot for source A25, envelope layer.}
   \label{fig:SgrB2-MErrorA25env}
\end{figure*}
\newpage
\clearpage




% core A26
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A26__env.pdf}\\
   \caption{Corner plot for source A26, envelope layer.}
   \label{fig:SgrB2-MErrorA26env}
\end{figure*}


% core A26
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A26__core.pdf}\\
   \caption{Corner plot for source A26, core layer.}
   \label{fig:SgrB2-MErrorA26core}
\end{figure*}
\newpage
\clearpage




% core A27
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-M/corner-triangle__SgrB2-M__A27__env.pdf}\\
   \caption{Corner plot for source A27, envelope layer.}
   \label{fig:SgrB2-MErrorA27env}
\end{figure*}
\newpage
\clearpage




==> figures/error/SgrB2-N/error-estimation__SgrB2-N.tex <==


%--------------------------------------------------------------------------------
% Error estimation of continuum parameters for cores in Sgr~B2(N)

    \subsection{Error estimation of continuum parameters for cores in Sgr~B2(N)}\label{app:ErrorSgrB2-N}

Corner plots \citepads{{corner}} showing the one and two dimensional projections of the posterior probability distributions of the continuum parameters of each core in Sgr~B2(N). On top of each column the probability distribution for each free parameter is shown together with the value of the best fit and the corresponding left and right errors. The left and right dashed lines indicate the lower and upper limits of the corresponding HPD interval, respectively. The dashed line in the middle indicates the mode of the distribution. The blue lines indicate the parameter values of the best fit. The plots in the lower left corner describe the projected 2D histograms of two parameters and the contours the HPD regions, respectively. In order to get a better estimation of the errors, we determine the error of the hydrogen column density and the emission measure on log scale and use the velocity offset (v$_{\rm off}$) related to the source velocity of v$_{\rm LSR}$ = 64~km~s$^{-1}$.


% core A01
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A01__env.pdf}\\
   \caption{Corner plot for source A01, envelope layer.}
   \label{fig:SgrB2-NErrorA01env}
\end{figure*}


% core A01
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.99\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A01__core.pdf}\\
   \caption{Corner plot for source A01, core layer.}
   \label{fig:SgrB2-NErrorA01core}
\end{figure*}
\newpage
\clearpage




% core A02
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A02__env.pdf}\\
   \caption{Corner plot for source A02, envelope layer.}
   \label{fig:SgrB2-NErrorA02env}
\end{figure*}


% core A02
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A02__core.pdf}\\
   \caption{Corner plot for source A02, core layer.}
   \label{fig:SgrB2-NErrorA02core}
\end{figure*}
\newpage
\clearpage




% core A03
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A03__env.pdf}\\
   \caption{Corner plot for source A03, envelope layer.}
   \label{fig:SgrB2-NErrorA03env}
\end{figure*}


% core A03
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A03__core.pdf}\\
   \caption{Corner plot for source A03, core layer.}
   \label{fig:SgrB2-NErrorA03core}
\end{figure*}
\newpage
\clearpage




% core A04
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A04__env.pdf}\\
   \caption{Corner plot for source A04, envelope layer.}
   \label{fig:SgrB2-NErrorA04env}
\end{figure*}


% core A04
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A04__core.pdf}\\
   \caption{Corner plot for source A04, core layer.}
   \label{fig:SgrB2-NErrorA04core}
\end{figure*}
\newpage
\clearpage




% core A05
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A05__env.pdf}\\
   \caption{Corner plot for source A05, envelope layer.}
   \label{fig:SgrB2-NErrorA05env}
\end{figure*}


% core A05
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A05__core.pdf}\\
   \caption{Corner plot for source A05, core layer.}
   \label{fig:SgrB2-NErrorA05core}
\end{figure*}
\newpage
\clearpage




% core A06
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A06__env.pdf}\\
   \caption{Corner plot for source A06, envelope layer.}
   \label{fig:SgrB2-NErrorA06env}
\end{figure*}


% core A06
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A06__core.pdf}\\
   \caption{Corner plot for source A06, core layer.}
   \label{fig:SgrB2-NErrorA06core}
\end{figure*}
\newpage
\clearpage




% core A07
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A07__env.pdf}\\
   \caption{Corner plot for source A07, envelope layer.}
   \label{fig:SgrB2-NErrorA07env}
\end{figure*}


% core A07
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A07__core.pdf}\\
   \caption{Corner plot for source A07, core layer.}
   \label{fig:SgrB2-NErrorA07core}
\end{figure*}
\newpage
\clearpage




% core A08
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A08__env.pdf}\\
   \caption{Corner plot for source A08, envelope layer.}
   \label{fig:SgrB2-NErrorA08env}
\end{figure*}
\newpage
\clearpage




% core A09
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A09__env.pdf}\\
   \caption{Corner plot for source A09, envelope layer.}
   \label{fig:SgrB2-NErrorA09env}
\end{figure*}


% core A09
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A09__core.pdf}\\
   \caption{Corner plot for source A09, core layer.}
   \label{fig:SgrB2-NErrorA09core}
\end{figure*}
\newpage
\clearpage




% core A10
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A10__env.pdf}\\
   \caption{Corner plot for source A10, envelope layer.}
   \label{fig:SgrB2-NErrorA10env}
\end{figure*}
\newpage
\clearpage




% core A11
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A11__env.pdf}\\
   \caption{Corner plot for source A11, envelope layer.}
   \label{fig:SgrB2-NErrorA11env}
\end{figure*}
\newpage
\clearpage




% core A12
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A12__env.pdf}\\
   \caption{Corner plot for source A12, envelope layer.}
   \label{fig:SgrB2-NErrorA12env}
\end{figure*}
\newpage
\clearpage




% core A13
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A13__env.pdf}\\
   \caption{Corner plot for source A13, envelope layer.}
   \label{fig:SgrB2-NErrorA13env}
\end{figure*}
\newpage
\clearpage




% core A14
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A14__env.pdf}\\
   \caption{Corner plot for source A14, envelope layer.}
   \label{fig:SgrB2-NErrorA14env}
\end{figure*}


% core A14
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A14__core.pdf}\\
   \caption{Corner plot for source A14, core layer.}
   \label{fig:SgrB2-NErrorA14core}
\end{figure*}
\newpage
\clearpage




% core A15
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A15__env.pdf}\\
   \caption{Corner plot for source A15, envelope layer.}
   \label{fig:SgrB2-NErrorA15env}
\end{figure*}


% core A15
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A15__core.pdf}\\
   \caption{Corner plot for source A15, core layer.}
   \label{fig:SgrB2-NErrorA15core}
\end{figure*}
\newpage
\clearpage




% core A16
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A16__env.pdf}\\
   \caption{Corner plot for source A16, envelope layer.}
   \label{fig:SgrB2-NErrorA16env}
\end{figure*}


% core A16
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A16__core.pdf}\\
   \caption{Corner plot for source A16, core layer.}
   \label{fig:SgrB2-NErrorA16core}
\end{figure*}
\newpage
\clearpage




% core A17
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A17__env.pdf}\\
   \caption{Corner plot for source A17, envelope layer.}
   \label{fig:SgrB2-NErrorA17env}
\end{figure*}


% core A17
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A17__core.pdf}\\
   \caption{Corner plot for source A17, core layer.}
   \label{fig:SgrB2-NErrorA17core}
\end{figure*}
\newpage
\clearpage




% core A18
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A18__env.pdf}\\
   \caption{Corner plot for source A18, envelope layer.}
   \label{fig:SgrB2-NErrorA18env}
\end{figure*}


% core A18
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A18__core.pdf}\\
   \caption{Corner plot for source A18, core layer.}
   \label{fig:SgrB2-NErrorA18core}
\end{figure*}
\newpage
\clearpage




% core A19
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A19__env.pdf}\\
   \caption{Corner plot for source A19, envelope layer.}
   \label{fig:SgrB2-NErrorA19env}
\end{figure*}


% core A19
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A19__core.pdf}\\
   \caption{Corner plot for source A19, core layer.}
   \label{fig:SgrB2-NErrorA19core}
\end{figure*}
\newpage
\clearpage




% core A20
\begin{figure*}[!htb]
   \centering
   \includegraphics[width=0.50\textwidth]{figures/error/SgrB2-N/corner-triangle__SgrB2-N__A20__env.pdf}\\
   \caption{Corner plot for source A20, envelope layer.}
   \label{fig:SgrB2-NErrorA20env}
\end{figure*}
\newpage
\clearpage



